MiME: Multilevel Medical Embedding of Electronic Health Records for Predictive Healthcare

Deep learning models exhibit state-of-the-art performance for many predictive healthcare tasks using electronic health records (EHR) data, but these models typically require training data volume that exceeds the capacity of most healthcare systems. External resources such as medical ontologies are used to bridge the data volume constraint, but this approach is often not directly applicable or useful because of inconsistencies with terminology. To solve the data insufficiency challenge, we leverage the inherent multilevel structure of EHR data and, in particular, the encoded relationships among medical codes. We propose Multilevel Medical Embedding (MiME) which learns the multilevel embedding of EHR data while jointly performing auxiliary prediction tasks that rely on this inherent EHR structure without the need for external labels. We conducted two prediction tasks, heart failure prediction and sequential disease prediction, where MiME outperformed baseline methods in diverse evaluation settings. In particular, MiME consistently outperformed all baselines when predicting heart failure on datasets of different volumes, especially demonstrating the greatest performance improvement (15% relative gain in PR-AUC over the best baseline) on the smallest dataset, demonstrating its ability to effectively model the multilevel structure of EHR data.

==> old_method.tex <==

In this section, we first describe the structure of EHR data.
Next we introduce the notations we will use in the \mname embedding, then describe the \mname framework.

% \subsection{EHR Data Modeling}
% \label{ssec:ehr_modeling}

% In most EHR systems, data are stored in relational databases, where tables containing information about patient demographics, encounters, medication orders and procedure orders are linked using keys such as \textit{patient ID}, \textit{encounter ID} or \textit{medication order ID}. Although there is more than one way to view EHR data, when performing computational tasks such as disease prediction, we typically group all information by individual patients as depicted by Figure~\ref{fig:ehr_graph}.

In most EHR systems, EHR data can be seen as a collection of individual patient records, where each patient has a sequence of encounters over time. 
Within an encounter, different types of events are intertwined via the clinical decision making process.
Typically, a patient is first diagnosed by a physician, which generates a set of diagnosis codes.
Then the physician can order medications or procedures based on the diagnosis, which generates a set of medication codes and procedure codes. 
Therefore, there is an explicit, perhaps causal, relationship between diagnosis codes and medication/procedure codes, as depicted by Figure~\ref{fig:ehr_graph}.

\begin{figure}[t]
\centering
\includegraphics[width=.7\textwidth]{figs/ehr_graph}
\caption{A visit record of a single patient. Red denotes diagnosis codes, and blue denotes medication/procedure codes. A visit is not merely a set of codes, but rather a hierarchically structured codes with heterogeneous relations.
For example, while both \textit{Acetaminophen} and \textit{IV fluid} form an explicit relationship with \textit{Fever}, they also are correlated with each other as children of \textit{Fever}.}
%\js{Fig 1 may need to connect to the notation somehow. Right now, they are messy in itself, I know we want to highlight the complexity of real-world EHR, but for the sake this paper, we probably want to show an abstract version which accurately represent the model. e.g., all the start and end dates, instruction, notes, QRS are irrelevant for this paper, and binary, continuous and text are not relevant either. }
%}
\label{fig:ehr_graph}
\end{figure}

In order to leverage deep learning's ability to learn complex features from input data, the EHR data must be transformed into a vector.
A patient can be seen as a sequence of visits (\textit{i.e.} encounters), and the visit sequence can be transformed into a vector using recurrent neural networks (RNN)~\cite{elman1990} or convolutional neural networks (CNN)~\cite{LeCun:2004:LMG:1896300.1896315,krizhevsky2012imagenet}.
However, transforming a visit to a vector leaves some room for imagination as it has a multilevel structure with inter-code relationships.
A typical approach adopted by a number of previous works~\cite{choi2016using, choi2016doctor, choi2016retain, choi2017gram, ma2017dipole, bajor2016predicting} flattens all events within a visit and represents it as a vector of individual features, losing the structural information embedded in the visit.
In this work, \mname focuses on the internal structure information of EHR data, and explicitly captures the heterogeneous relationships between the diagnosis codes and the medication/procedure codes.
Although we focus on diagnosis codes and medication/procedures codes in this work, the proposed methodology \mname can be applied to model other relations in EHR data as well. 

\subsection{Notations of \mname}
\begin{table}[t]
\caption{Notations for \mname}
\label{table:notation}
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{c|l}
\hline
\bf Notation & \bf  Definition  \\
\hline
\hline
$\mathcal{A}$ & Set of all diagnosis codes.\\
$\mathcal{B}$ & Set of all treatment (medications and procedures) codes.\\
$\mathcal{V}^{{(t)}}$ & A patient's $t$-th hospital visit. It is a set of diagnosis objects $\mathcal{O}^{(t)}_0, \mathcal{O}^{(t)}_1, \ldots$.\\
$\vb^{(t)}$ & A vector representation of $\mathcal{V}^{(t)}$.\\
$\mathcal{O}^{(t)}_{i}$ & $i$-th diagnosis object of $t$-th hospital visit.\\
 & It contains a single diagnosis code $d_{i}^{(t)} \in \mathcal{A}$ and the associated treatment codes $\mathcal{M}_{i}^{(t)}$.\\
$\ob^{(t)}_{i}$ & A vector representation of $\mathcal{O}^{(t)}_{i}$.\\
%$d_{i}^{(t)}$ & Diagnosis code of $\mathcal{D}^{(t)}_{i}$ which is an element of $\mathcal{A}$\\
%$\mathcal{M}_{i}^{(t)}$ & A set of treatment codes a patient received for $d_{i}^{(t)}$\\
$m_{i,j}^{(t)}$ & $j$-th treatment code of $\mathcal{M}_{i}^{(t)}$. It is an element of $\mathcal{B}$.\\
$g(d_{i}^{(t)}, m_{i,j}^{(t)})$ & A function that captures the interaction between $d_{i}^{(t)}$ and $m_{i,j}^{(t)}$.\\
$f(d_{i}^{(t)}, \mathcal{M}_{i}^{(t)})$ & A function that derives $\ob^{(t)}_{i}$.\\
%$f(\mathcal{O}_{i}^{(t)})$ & A function that generates $\ob^{(t)}_{i}$.\\
$r(\cdot)$ & A function that retrieves $d_{i}^{(t)}$ or $m_{i,j}^{(t)}$'s embedding vector.\\
\hline
\end{tabular}
\end{table}

Notations we will use throughout the paper are described in Table~\ref{table:notation}.
Let's assume a patient makes a sequence of visits $\mathcal{V}^{(1)}, \mathcal{V}^{(2)}, \ldots, \mathcal{V}^{(t)}$ over time.
Each visit $\mathcal{V}^{(t)}$ contains a varying number of diagnosis (Dx) objects $\mathcal{O}_{1}^{(t)}, \mathcal{O}_{2}^{(t)}, \ldots, \mathcal{O}_{|\mathcal{V}^{(t)}|}^{(t)}$, where each $\mathcal{O}_{i}^{(t)}$ consists of a single Dx code $d_{i}^{(t)} \in \mathcal{A}$ and a set of associated treatments (medications or procedures) $\mathcal{M}_{i}^{(t)}$, which in turn consists of treatment codes $m_{i,1}^{(t)}, m_{i,2}^{(t)}, \ldots, m_{i,|\mathcal{M}_{i}^{(t)}|}^{(t)} \in \mathcal{B}$.
To reduce clutter, we omit the superscript $(t)$ indicating $t$-th visit, when we are discussing a single visit.

In Figure~\ref{fig:ehr_graph}, there are five Dx codes, hence five Dx objects.
If we count from leftmost Dx (\textit{Fatigue}) to the rightmost Dx (\textit{Chest paint}), the first Dx object $\mathcal{O}_{1}$ has \textit{Fatigue} as the Dx code, but no treatment codes.
$\mathcal{O}_{2}$, on the other hand, has \textit{Cough} as the Dx code and two associated treatment codes, \textit{Benzonatate} and \textit{Acetaminophen}.
In such cases, we can use $g(\cdot, \cdot)$ to capture the interaction between a Dx code and a treatment code, which will be fed to $f(\cdot)$ to obtain the vector representation of a Dx object.
Figure~\ref{fig:model} depicts the overall process of our approach, further details will be described in the following section.
%Each diagnosis code $d_{t,i}$ can be associated with one or more medication codes $m_{t,i,0}, m_{t,i,1} \ldots, m_{t,i,|m_{t,i}|} \in \mathcal{M}$ and one or more procedure codes $p_{t,i,0}, p_{t,i,1} \ldots, p_{t,i,|p_{t,i}|} \in \mathcal{P}$ where $\mathcal{M}$ and $\mathcal{P}$ respectively denote the set of unique medication codes and the set of unique procedure codes in the data.
%$|m_{t,i}|$ and $|p_{t,i}|$ respectively denote the total number of medication codes and procedure codes associated with $d_{t,i}$.
As shown by Figure~\ref{fig:ehr_graph}, some treatment codes (\textit{e.g. Acetaminophen}) can be shared by two or more Dx codes (\textit{e.g. Cough, Fever}), if the doctor ordered a single medication for more than one diagnosis.
In that case, each Dx object will have its own copy of the treatment code attached to it.

\subsection{Description of \mname}
\label{ssec:model_description}
\begin{figure}[ht]
\centering
\includegraphics[width=0.85\textwidth]{figs/FLOW2.png}
\caption{Prediction model using \mname. Medical codes are embedded into multiple levels: diagnosis-level, visit-level, and patient-level. Final prediction $p(\yb|\hb)$ is based on the patient representation $\hb$, which is derived from visit representations $\vb^{(0)}, \vb^{(1)}, \ldots$, where each $\vb^{(t)}$ is generated using \mname framework. \ecedit{Talk about capturing interaction and auxiliary task.}
%\js{this figure needs to be simplified, and contain notations, maybe we don't need fig 1 at all}
}
\label{fig:model}
\end{figure}

As discussed earlier, previous approaches often flatten the EHR structure such that Dx codes and treatment codes are packed in the same vector.
Then a single visit $\mathcal{V}^{(t)}$ can be expressed as a binary vector $\xb^{(t)} \in \{0,1\}^{|\mathcal{A}| + |\mathcal{B}|}$ where each dimension corresponds to a specific Dx and treatment code.
Therefore encoding a sequence of visits made by a patient was achieved as follows:
\begin{align*}
\vb^{(t)} & = \sigma(\Wb_x \xb^{(t)}) \\
\hb & = h(\vb^{(1)}, \vb^{(2)}, \ldots, \vb^{(t)})
\end{align*}
where $\Wb_x$ is the embedding matrix that converts the binary vector $\xb$ to a lower-dimensional visit representation\footnote{We omit bias variables throughout the paper to reduce clutter.}, $\sigma$ a non-linear activation function such as sigmoid or rectified linear unit (ReLU), $h(\cdot)$ a function that maps a sequence of visit representations $\vb^{(0)}, \ldots, \vb^{(t)}$ to a patient representation $\hb$. $h(\cdot)$ can be simply an RNN or a complex combination of RNNs and CNN and attention mechanisms~\cite{bahdanau2014neural}.\js{maybe we can experiment with all 3 RNN, CNN and attention}
\ecedit{Justification for using RNN in the experiments: We want to minimize the expressivity of $h(\cdot)$ so that the effect of visit embedding can be properly evaluated.}

\mname treats the Dx codes $\mathcal{A}$ and the treatment codes $\mathcal{B}$ separately, in order to capture the relationship between $\mathcal{A}$ and $\mathcal{B}$ depicted by Figure~\ref{fig:ehr_graph}.
Then a single visit $\mathcal{V}$ (omitting the index $(t)$ of the visit) consists of two levels: the diagnosis level, and the treatment level.
Figure~\ref{fig:model} illustrates how the proposed model \mname builds the representation of $\mathcal{V}$ in a bottom-up fashion and how we capture both co-occurrence and parent-child relationship among the codes in Figure~\ref{fig:ehr_graph} via multilevel embedding.
In a single Dx object $\mathcal{O}_i$, a Dx code $d_i$ and its associated treatment codes $\mathcal{M}_i$ are used to obtain a vector representation of $\mathcal{O}_i$, $\ob_i$.
%\footnote{Diagnosis embedding $\db_i$, which is vector representation of a diagnosis code and its associated medication/procedure codes,  is not to be confused with a diagnosis code embedding which is vector representation of a single diagnosis code $d_i$}.
Then multiple Dx object embeddings $\ob_0, \ldots, \ob_{|\mathcal{V}|}$ in a single visit are used to obtain a visit embedding $\vb$, which in turn forms a patient embedding $\hb$ with other visit embeddings.
%As shown in Figure~\ref{fig:model}, we also aim to capture the interactions between a diagnosis code and its associated medication codes and procedure codes, in order to obtain a more accurate diagnosis embedding.
The skeletal form of \mname is as follows,
\begin{align}
%\vb & = \sum_{i}^{|d|} \db_i \label{eq:skelenton}\\
%\db_i & = f_d \Big( d_i, \sum_{j}^{|m_i|} \mb_{i,j}, \sum_{k}^{|p_i|} \pb_{i,k} \Big) \label{eq:skelenton} \\
%\mb_{i,j} & =  f_{d,m} (d_i, m_{i,j})\\
%\db_i & = f_d \Big( d_i, \sum_{j}^{|m_i|} f_{d,m} (d_i, m_{i,j}), \sum_{k}^{|p_i|} f_{d,p} (d_i, p_{i,k}) \Big) \nonumber \\
%\vb & = \sigma \Big( \sum_{i}^{|\mathcal{V}|} f(d_i, \mathcal{M}_i) \Big) \label{eq:skelenton} \\
\vb & = \sigma \Big( \sum_{i}^{|\mathcal{V}|} \underbrace{f ( d_i, \mathcal{M}_i ) \Big)}_{\text{Diagnosis object embedding $\ob_i$}} \label{eq:skelenton} \\
f(d_i, \mathcal{M}_i) & = \ob_i = \Ub \bigg( r(d_i) + \sigma \Big( \sum_{j}^{|\mathcal{M}_i|} g(d_i, m_{i,j}) \Big) \bigg) \\
g(d_i, m_{i,j}) & = \Wb r(d_i) \odot r(m_{i,j}))
%|m_i| & : \mbox{\footnotesize The number of medication orders associated with the $i$-th diagnosis } d_i \nonumber \\
%f_{d,m}(\cdot, \cdot) & : \mbox{\footnotesize Function that captures the relationship between a diagnosis} \nonumber \\[-5pt]
%& \mbox{\quad \footnotesize and a medication order.} \nonumber \\[-2pt]
%|p_i| & : \mbox{\footnotesize The number of procedure orders associated with the $i$-th diagnosis } d_i \nonumber \\
%f_{d,p}(\cdot, \cdot) & : \mbox{\footnotesize Function that captures the relationship between a diagnosis} \nonumber \\[-5pt]
%& \mbox{\quad \footnotesize and a procedure order.} \nonumber \\[-2pt]
%|d| & : \mbox{\footnotesize The number of diagnoses in the visit } \mathcal{V}. \nonumber \\
%f_d(\cdot, \cdot, \cdot) & : \mbox{\footnotesize Function that generates a single diagnosis embedding $\db_i$.} \nonumber
\end{align}

%In this work we propose two versions of \mname and conduct experiments with both models. The first version, $\mname_{sum}$ implements the functions $f_d, f_{d,m}$ and $f_{d,p}$ as follows:
%\begin{align}
%f_{d,m}(d_i, m_{i,j}) & = \eb_m(m_{i,j}) \nonumber \\
%f_{d,m}(d_i, m_{i,j}) & = f_{rx}(m_{i,j}) = \sigma(\W_{rx} \mb_{i,j}) \nonumber \\
%f_{d,p}(d_i, p_{i,k}) & = f_{pr}(p_{i,k}) = \sigma(\W_{pr} \pb_{i,k})\nonumber \\
%f_{d,m}(d_i, m_{i,j}) & = f_{rx}(m_{i,j}) \nonumber \\
%f_{d,p}(d_i, p_{i,k}) & = f_{pr}(p_{i,k})\nonumber \\
%& f_d \Big( d_i, \sum_{j}^{|m_i|} f_{d,m} (d_i, m_{i,j}), \sum_{k}^{|p_i|} f_{d,p} (d_i, p_{i,k}) \Big) = \nonumber \\
%f_{d}(\cdot, \cdot, \cdot) = \db_i & = \sigma \bigg( \Wb_d \Big( \eb_d(d_i) + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j) \Big) \bigg) \nonumber
%f_{d}(\cdot, \cdot, \cdot) = \db_i & = \sigma \bigg( \Wb_d \Big( f_{dx}(d_i) + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j) \Big) \bigg) \nonumber
%\mbox{where } f_{dx}(d_i) = \sigma(\W_{dx} \db_{i})
%\end{align}
where $f_{dx}(\cdot), f_{rx}(\cdot)$ and $f_{pr}(\cdot)$ respectively denote the embedding functions that map given diagnosis, medication, and procedure codes to their corresponding vector representations.
In \mname$_{sum}$, the size of all code embeddings are the same as they are summed to obtain the diagnosis embedding $\db_i$.
%\js{all these $\eb_d, \eb_m$ and $\eb_p$ are functions in your notation, so let's describe them that way, in particular, explain the output of the function and the sizes of the output. it seems to require the same size for all e?}
$\Wb_d$ is the weight matrix used to obtain the representation of a single diagnosis object, which is applied to the sum of diagnosis code embedding $f_{dx}(d_i)$ and its associated medication/procedure code embeddings $f_{rx}(m_{i,j})$ and $f_{pr}(p_{i,k})$. $\sigma$ is the non-linear activation function, for which we used ReLU in this work.
In $\mname_{sum}$, the functions $f_{d,m}(\cdot, \cdot)$ and $f_{d,m}(\cdot, \cdot)$, which aim to capture the interactions between a diagnosis code and medication/procedure codes are simply implemented as a medication code embedding $f_{rx}(m_{i,j})$ and a procedure code embedding $f_{pr}(p_{i,k})$.
In $\mname_{sum}$, it is assumed that the code interactions are implicitly captured by the summation inside the diagnosis embedding generator $f_d(\cdot, \cdot, \cdot)$.
Although this is a rather straightforward implementation of Eq.~\ref{eq:skelenton}, it shows robust performance in various prediction tasks as we will demonstrate in the next section.

The second implementation of Eq.~\ref{eq:skelenton}, which we name $\mname_{bp}$, captures the relationship between the diagnosis code and medication/procedure orders more explicitly as follows:
\small
\begin{align}
f_{d,m}(d_i, m_{i,j}) & = \sigma(\Wb_{dm} f_{dx}(d_i) \odot f_{rx}(m_{i,j})) \nonumber \\
f_{d,p}(d_i, p_{i,k}) & = \sigma(\Wb_{dp} f_{dx}(d_i) \odot f_{pr}(p_{i,k})) \nonumber 
\\
f_{d}(\cdot, \cdot, \cdot) = \db_i & = \sigma \bigg( \Wb_d \Big( f_{dx}(d_i) + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j) \Big) \bigg) \nonumber
%& f_d \Big( d_i, \sum_{j}^{|m_i|} f_{d,m} (d_i, m_{i,j}), \sum_{k}^{|p_i|} f_{d,p} (d_i, p_{i,k}) \Big) = \nonumber \\
%& \sigma \bigg( \Wb_d \Big( \eb_d(d_i) + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j) \Big) \bigg) \nonumber
\end{align}
\normalsize
Both $f_{d,m}$ and $f_{d,p}$ use a form of bilinear pooling to explicitly capture the interactions between the diagnosis code and medication/procedure codes.
%\js{we should explicitly and mathematically define bilinear pooling}
Bilinear pooling~\cite{tenenbaum12emph} derives a scalar feature $f_i$ between two embeddings $\xb, \yb$ such that $f_i = \xb^T \Wb_i \yb$ where $\Wb_i$ is a trainable weight matrix.
Since we typically extract many features $f_0, \ldots, f_i$, to capture the interaction between two embeddings, bilinear pooling requires us to train a number of weight matrices (\textit{i.e.} weight tensor).
%is typically used to capture the interaction between two different embeddings,
Due to the large number of parameters required, researchers developed more efficient methods such as compact bilinear pooling~\cite{gao2016compact,fukui2016multimodal} and low-rank bilinear pooling~\cite{kim2016hadamard}.
In this work, we used a simplified version of low-rank bilinear pooling with Hadamard product~\cite{kim2016hadamard}, which showed impressive performance in Visual Question Answering (VQA), where it is important to effectively capture the interaction between two different domains:text-based question and  image.
Weight matrices $\Wb_{dm}$ and $\Wb_{dp}$ are used to send the diagnosis code embedding $f_{dx}(d_i)$ into another latent space, where the interaction between diagnosis $d_i$ and the corresponding $m_{i,j}$ (or procedure $p_{i,k}$) can be captured effectively.
In $\mname_{bp}$ the interactions captured by $f_{d,m}$ and $f_{d,p}$ are added to the diagnosis code embedding $f_{dx}(d_i)$, which can be interpreted as adjusting the diagnosis representation according to its associated medication and procedure orders
\footnote{For both $\mname_{sum}$ and $\mname_{bp}$, we also implemented $f_d$ as a concatenation of $f_{dx}(d_i), \sum f_{d,m}$ and $\sum f_{d,p}$ instead of a summation, but it showed slightly weaker performance.}.

\subsection{Joint Training with Auxiliary Tasks}
\label{ssec:method_auxiliary}
\js{I doubt reviewers have read this section as they are all confused with the notations, let's make sure we clean up this as well}
Since the expressive power of deep learning models comes from their large number of parameters in multiple layers, they typically require a large amount of training data. This poses a challenge in deep embedding tasks on smaller datasets, which are often the case in new EHR systems, with a small number of patients each with a relatively fewer number of visits.
In such cases, to prevent the deep models from over-fitting, we adopt a multi-task learning (MTL) approach that can inductively transfer the knowledge contained in multiple auxiliary prediction tasks to improve the model's generalization performance on the original prediction task.
%given that we choose auxiliary tasks that are related to the original task.
MTL was shown to improve model robustness in medical concept embedding.
For example, in ~\cite{suo_amia_mtl}, multiple severity status of a disease were seen as multiple tasks for improving accuracy in disease prediction.
%\begin{figure}[t]
%\centering
%\includegraphics[width=1.\textwidth]{figs/mtl.png}
%\caption{Diagnosis embedding and its associated auxiliary prediction tasks, where Dx prediction, Rx prediction, and Procedure prediction serve as auxiliary tasks for improving the performance of some specific target task.\js{same comment: notation should be part of this, and simplify the figure, no point of have 3 branches all in details}}
%\label{fig:mtl_model}
%\end{figure}

For deep learning models which are typically composed of layers of neurons, an MTL strategy can require certain neurons to be shared among all tasks, and certain neurons to be specialized for specific tasks ~\cite{caruana1998multitask}.
Specifically, in longitudinal EHR data based health analytics, the patient embedding $\hb$ is typically used for specific prediction tasks, such as heart failure prediction or mortality prediction.
And the representation power of $\hb$ comes from properly capturing each visit $\mathcal{V}_t$, and modeling the longitudinal aspect with the function $f(\vb_0, \ldots, \vb_t)$.
Since the focus of this work is on modeling a single visit $\mathcal{V}_t$, our MTL strategy performs auxiliary tasks while obtaining the $t$-th visit embedding $\vb_t$ as follows.
\small
\begin{align*}
%& \db_i = \sigma \bigg( \Wb_d \Big( \eb_d(d_i) + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j) \Big) \bigg)\\
& \vb_t = \sum_{i}^{|d_t|} \db_{t,i} \\
& \hat{d}_{t,i} = p(d_{t,i} | \db_{t,i}) = \mbox{softmax}(\Wb_{ad} \db_{t,i}) \\
& \hat{\mb}_{t,i} = p(\mb_{t,i} | \db_{t,i}) = \sigma (\Wb_{am} \db_{t,i}) \\
%p(m_{i,0}, \ldots, m_{i, |m_i|} | \db_i) & = \sigma (\Wb_{am} \db_i) \\
& \hat{\pb}_{t,i} = p(\pb_{t,i} | \db_{t,i}) = \sigma (\Wb_{ap} \db_{t,i})\\
& L_{aux} = -\lambda_{aux} \sum_{t}^{T} \Big( CE(d_{t,i}, \hat{d}_{t,i}) + CE(\mb_{t,i}, \hat{\mb}_{t,i}) + CE(\pb_{t,i}, \hat{\pb}_{t,i}) \Big)
%p(p_{i,0}, \ldots, p_{i, |p_i|} | \db_i) & = \sigma (\Wb_{ap} \db_i)
\end{align*}
\normalsize
Given diagnosis embeddings $\db_{t,0}, \ldots, \db_{t,|d_t|}$, before aggregating them to obtain $\vb_t$, the model predicts the diagnosis code $d_{t,i}$, and the associated medication codes $\mb_{t,i} = m_{t,i,0}, \ldots$, $m_{t,i,|m_{t,i}|}$ and procedure codes $\pb_{t,i} = p_{t,i,0}, \ldots, p_{t,i,|p_{t,i}|}$, involved with $\db_{t,i}$.
$\Wb_{ad}, \Wb_{am}$ and $\Wb_{ap}$ are weight matrices used for predicting the diagnosis, medication and procedure code, respectively.
$CE(\cdot, \cdot)$ denotes the cross-entropy function, and $\lambda_{aux}$ is the coefficient for the auxiliary loss term.
We used the softmax function for predicting $d_{t,i}$ since in a single diagnosis embedding, there is only one diagnosis code involved.
However, there could be no medication/procedure codes associated with $d_{t,i}$, and therefore we used the sigmoid function for predicting medication and procedure codes.

These auxiliary tasks guide the model to learn diagnosis embeddings $\db_{t,i}$ that are representative of the specific codes involved with it. 
Correctly capturing the events within an encounter is a foundation of all downstream prediction tasks, and these general-purpose auxiliary tasks, combined with the specific target task, encourage the model to learn visit embeddings $\vb_t$ that are not only tuned for the target prediction task, but also grounded in general-purpose foundational knowledge.

% \iffalse
% \subsection{Attention pooling}
% In the previous section, the way we dealt with multiple number of medication orders (\textit{i.e.} medication codes) $m_{i,0}, m_{i,1}, \ldots$ that are associated with the $i$-th diagnosis $d_i$ was to obtain a representation for individual medication order and add them all such that $\sum_{j}^{|m_i|} f_{d,m} (d_i, m_{i,j})$. The same principle was applied to the procedure orders $p_{i,0}, p_{i,1}, \ldots$ associated with $d_i$. 
% Identically, the way we pooled information from multiple diagnoses $d_0, d_1, \ldots$ in a visit $\mathcal{V}$ was to sum the diagnosis object representations such that $\sum_{i}^{|d|} f_d(d_i, \cdot, \cdot)$. 

% However, we can replace the simple summation with the attention mechanism~\cite{bahdanau2014neural} to pool information from multiple medication/procedure orders and diagnosis objects so that \mname can intelligently select important medication/procedure orders and diagnosis objects that have a high correlation with the prediction target. We can rewrite the skeletal form of \mname in Eq.~\ref{eq:skelenton} to incorporate attention mechanism as follows:
% \begin{align}
% \vb & = \sum_{i}^{|d|} \alpha_i f_d \Big( d_i, \sum_{j}^{|m_i|} \beta_{i,j} f_{d,m} (d_i, m_{i,j}), \sum_{k}^{|p_i|} \gamma_{i,k} f_{d,p} (d_i, p_{i,k}) \Big) \label{eq:attention} \\
% \bm{\beta}_i & = \mbox{softmax} \big( f_{\beta}(m_{i,0}), \ldots, f_{\beta}(m_{i,|m_i|} \big) \nonumber \\
% \bm{\gamma}_i & = \mbox{softmax} \big( f_{\gamma}(p_{i,0}), \ldots, f_{\gamma}(p_{i,|p_i|} \big) \nonumber \\
% \bm{\alpha} & = \mbox{softmax} \big( f_{\alpha}(d_0, \mb_0, \pb_0), \ldots, f_{\alpha}(d_{|d|}, \mb_{|d|}, \pb_{|d|}) \big) \nonumber
% \end{align}
% where $\mb_i$ and $\pb_i$ denotes all medication codes and procedure codes associated with the $i$-th diagnosis, respectively. $f_{\alpha}, f_{\beta}$ and $f_{\gamma}$ are functions that generate unnormalized attentions respectively for diagnosis objects, medication orders and procedure orders, and they are typically implemented as a multilayer perceptron (MLP) with a scalar output whose range is $-\infty \sim \infty$.

% Eq.~\ref{eq:attention} can be seen as a generalized version of Eq.~\ref{eq:skelenton}. If all attention weights $\bm{\alpha}, \bm{\beta}_i$ and $\bm{\gamma}_i$ are always fixed to $\mathbf{1}$, then Eq.~\ref{eq:attention} becomes equivalent to Eq.~\ref{eq:skelenton}. Employing attention mechanism can help obtain extra performance improvement, but in also provides insight into the inner-workings of the deep learning model. This model interpretability is an important aspect especially in healthcare, and attention mechanism has been successfully combined with neural network models in computational healthcare for providing interpretation to the model behavior~\cite{choi2016retain,choi2017gram,ma2017dipole}. In this work, as a proof-of-concept, we apply attention mechanism on the diagnosis level (\textit{i.e.} $\bm{\alpha}$) and demonstrate its outcome in the experiments.
% \fi

%where $|d|$ is the total number of diagnoses in $\mathcal{V}$, 
%\vb & = \sum_{i}^{|d|} \sigma \bigg( \Wb_d \Big( \db_i + \sum_{j}^{|m_i|} f_{d,m} (d_i, m_j) + \sum_{k}^{|p_i|} f_{d,p} (d_i, p_j)\\
%\sigma ( \Wb_m \mb_j) + \sum_{k}^{|p_i|} \sigma ( \Wb_p \pb_k) \Big) \bigg)\\
%\Wb_m & = f_m(\db_i) \mbox{ or } f_m(\db_i, \hb_{t-1})\\
%\Wb_p & = f_p(\db_i) \mbox{ or } f_p(\db_i, \hb_{t-1})\\
%\hb_t & = RNN(\vb_0, \vb_1, \ldots, \vb_t)
%$\Wb_m$ and $\Wb_p$ are conditionally generated based on the diagnosis code in order to capture the causal relationship between the diagnosis code and the medication/procedure orders. 

%In order to facilitate model interpretation, we can replace the simple summations with attention mechanism s as follows:
%\begin{align*}
%\vb_t & = \sum^{\db} \alpha_i \sigma \bigg( \Wb_d \Big( \db_i + \\
%& \sum^{\mb} \beta_i \sigma ( \Wb_m \mb_i) + \sum^{\pb} \gamma_i \sigma ( \Wb_p \pb_i) \Big) \bigg)\\
%\alpha_i & = f_{\alpha} (\db_i) \mbox{ or } f_{\alpha}(\db_i, \hb_{t-1})\\
%\beta_i & = f_{\beta} (\mb_i, \db_i) \mbox{ or } f_{\alpha}(\mb_i, \db_i, \hb_{t-1})\\
%\gamma_i & = f_{\gamma} (\pb_i, \db_i) \mbox{ or } f_{\alpha}(\pb_i, \db_i, \hb_{t-1})\\
%\Wb_m & = f_m(\db_i) \mbox{ or } f_m(\db_i, \hb_{t-1})\\
%\Wb_p & = f_p(\db_i) \mbox{ or } f_p(\db_i, \hb_{t-1})\\
%\hb_t & = RNN(\vb_0, \vb_1, \ldots, \vb_t)
%\end{align*}


%we constrain the heart failure prediction task accompanied with some specific auxiliary tasks having "shared common prior" with the focused heart failure prediction task. The simultaneous learning of focused and auxiliary tasks fully exploit the task relatedness and boost the prediction performance for the focused task. In particular, the auxiliary tasks we use include xxx ,and their formulations are given below.

==> oldold_method.tex <==
Given multiple data modalities $\xb_1, \xb_2, \ldots, \xb_n$, we want to correctly predict the label $\yb$. Formally put, we want to maximize the probability of $\log p(\yb | \xb_1, \xb_2, \ldots, \xb_n) = \log p(\yb | \Xb)$. Then we assume there is a true underlying patient state $\zb$, and incorporate it in $\log p(\yb | \Xb)$ as follows.
\begin{align}
\log p(\yb | \Xb) & = \log \int_z p(\yb, \zb | \Xb) dz \nonumber \\
& = \log \int_z p(\yb | \zb, \Xb) p(\zb | \Xb) dz \nonumber \\
& = \log \int_z p(\yb | \zb) p(\zb | \Xb) dz \nonumber \\%\mbox{ because $\zb$ is the true state, $\xb$ is redundant information for predicting $\yb$} \\
& = \log E_{\zb \sim p(\zb | \Xb)} [p(\yb | \zb)] \nonumber \\
& \ge E_{\zb \sim p(\zb | \Xb)} [\log p(\yb | \zb)] \label{eq:obj}
\end{align}
Now we need to maximize $\log p(\yb | \zb)$ and approximate $p(\zb | \Xb)$ at the same time. We plan to approximate $p(\zb | \Xb)$ with $q(\zb | \Xb)$ using variational autoencoder (VAE) technique. Specifically, minimizing $D_{KL} (q(\zb | \Xb) || p(\zb | \Xb))$ can be done by maximizing the evidence lower bound (ELBO).
\begin{align}
ELBO = E_q [\log p(\Xb | \zb)] - D_{KL} (q(\zb | \Xb) || p(\zb)) \label{eq:elbo}
\end{align}
We could first maximize Eq.\eqref{eq:elbo}, then separately maximize $\log p(\yb | \zb)$. However, this will not give us the true state $\zb$ that is useful for predicting $\yb$ because the optimization procedures for Eq.\eqref{eq:elbo} and $\log p(\yb | \zb)$ are disconnected.

How do we optimize Eq.\eqref{eq:obj} to satisfy the discussed criteria? So far we have two approaches.
\subsection{Power game between prediction and ELBO}
\begin{figure}
\centering
\includegraphics[scale=.5]{figs/model_1}
\caption{(Left) Maximizing $p(\yb | \zb)$. (Right) Maximizing ELBO using VAE}
\label{fig:model1}
\end{figure}
When maximizing $p(\yb | \zb)$, we can actually let the error signal flow from $\yb$ all the way to $\xb$, because we use the reparametrization trick between $\xb$ and $\zb$. Figure~\ref{fig:model1} shows the model architecture of both $p(\yb | \zb)$ and ELBO (VAE). Maximizing $p(\yb | \zb)$ in such a way will certainly shape $\zb$ in a way that is useful for prediction. However, it will destroy the distribution $q(\zb | \xb)$, thus destroying Eq.\eqref{eq:obj}. Therefore we must repeatedly maximize Eq.\eqref{eq:elbo} every now and then. 

\subsection{Double VAE}

==> tables/confusion_matrix.tex <==
\begin{table}[t]
\caption{Heart failure (HF) prediction performance in terms of false positive rate (FPR) and true positive rate (TPR). Models with significantly lower TPR values are grayed out as they have minimal value for HF prediction. 
\js{fix the error on TPR, btw this results are also not impressive, unless those numbers are all different}}
\hspace{-0.15in}
\label{table:confusion_matrix}
%\resizebox{\columnwidth}{!}{%
\centering
\small
\begin{tabular}{l|c|c}
& False positive rate & True positive rate\\
\hline
%raw &  0.8705 (0.0075) &  0.0176 (0.0067) &  0.0815 (0.0049) &  0.0304 (0.0042)\\
raw &  0.0176 (0.0067) &  0.0304 (0.0042)\\
%linear &  0.0186 (0.0066) & 0.0331 (0.0055)\\
linear &  0.0186 (0.0066) &  0.0331 (0.0055)\\
%sigmoid & 0.8758 (0.0035) &  \bf 0.0123 (0.0036) &  0.0874 (0.0052) &  0.0246 (0.0037)\\
%\textcolor{light_gray}{sigmoid} & \textcolor{light_gray}{0.8758 (0.0035)} & \textcolor{light_gray}{0.0123 (0.0036)} & \textcolor{light_gray}{0.0874 (0.0052)} & \textcolor{light_gray}{0.0246 (0.0037)}\\
\textcolor{light_gray}{sigmoid} & \textcolor{light_gray}{0.0123 (0.0036)} & \textcolor{light_gray}{0.0246 (0.0037)}\\
%relu &  0.8681 (0.0079) &  0.0199 (0.0075) &  0.0785 (0.0074) &  0.0334 (0.0064)\\
relu & 0.0199 (0.0075) & 0.0334 (0.0064)\\
%linear$_m$ & 0.8666 (0.0081) &  0.0215 (0.0086) &  0.0826 (0.0095) &  0.0294 (0.0083)\\
linear$_m$ & 0.0215 (0.0086) & 0.0294 (0.0083)\\
 %sigmoid$_m$ &  0.8734 (0.0035) &  0.0147 (0.0033) &  0.0871 (0.0047) &  0.0249 (0.0035)\\
%\textcolor{light_gray}{sigmoid$_m$} & \textcolor{light_gray}{0.8734 (0.0035)} & \textcolor{light_gray}{0.0147 (0.0033)} & \textcolor{light_gray}{0.0871 (0.0047)} & \textcolor{light_gray}{0.0249 (0.0035)}\\
\textcolor{light_gray}{sigmoid$_m$} & \textcolor{light_gray}{0.0147 (0.0033)} & \textcolor{light_gray}{0.0249 (0.0035)}\\
%relu$_m$ &  0.8666 (0.0036) &  0.0214 (0.0034) & 0.0789 (0.0069) &  0.0330(0.0051)\\
relu$_m$ & 0.0214 (0.0034) & 0.0330(0.0051)\\
 %sigmoid$_{mlp}$ &  0.8880 (0.0023) &  0 (0) &  0.1120 (0.0023) &  0 (0)\\
%\textcolor{light_gray}{sigmoid$_{mlp}$} & \textcolor{light_gray}{0.8880 (0.0023)} & \textcolor{light_gray}{0 (0)} & \textcolor{light_gray}{0.1120 (0.0023)} &  \textcolor{light_gray}{0 (0)}\\
\textcolor{light_gray}{sigmoid$_{mlp}$} & \textcolor{light_gray}{0 (0)} & \textcolor{light_gray}{0 (0)}\\
%relu$_{mlp}$ &  0.8709 (0.0029) &  0.0171 (0.0042) &  0.0820 (0.0068) & 0.0300 (0.0047)\\
relu$_{mlp}$ & 0.0171 (0.0042) & 0.0300 (0.0047)\\
%med2vec &  0.8666 (0.0044) &  0.0214 (0.0037) &  0.0814 (0.0050) &  0.0305 (0.0032)\\
med2vec & 0.0214 (0.0037) & 0.0305 (0.0032)\\
%$\mname_{sum}$ &  0.8702 (0.0027) &  0.0178 (0.0041) & 0.0795 (0.0083) &  0.0325 (0.0063)\\
$\mname_{sum}$ & 0.0178 (0.0041) & 0.0325 (0.0063)\\
%$\mname_{bp}$ &  0.8710 (0.0048) &  \textbf{0.0170} (0.0033) & 0.0779 (0.0039) & \textbf{0.0341} (0.0030)\\
$\mname_{bp}$ & \textbf{0.0170} (0.0033) & \textbf{0.0341} (0.0030)\\
\hline
\end{tabular}
\normalsize
\end{table}

==> tables/exp1_table_full_old.tex <==
\begin{table*}[ht]
\caption{HF prediction performance on small datasets. Values in the parentheses denote standard deviations from 5-fold random data splits. Two best values in each column are marked in bold.}
\label{table:exp1_full}
% \small
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{l|c|c|c|c|c|c}
 & \multicolumn{3}{c|}{\textbf{D$_1$ (Visit complexity 0-15\%, 5608 patients)}} & \multicolumn{3}{c}{\textbf{D$_3$ (Visit complexity 30-100\%, 5231 patients)}}\\
\hline
& test loss & test ROC-AUC & test PR-AUC & test loss & test ROC-AUC & test PR-AUC \\
\hline
raw & 0.2553 (0.0084) & 0.7424 (0.0153) & 0.2669 (0.0314) & 0.2144 (0.0127) & 0.8130 (0.0315) & 0.3776 (0.0589)\\
linear & 0.2562 (0.0108) & 0.7298 (0.0187) & 0.2722 (0.0354) & 0.2021 (0.0176) & 0.8209 (0.0130) & 0.4339 (0.0411)\\
sigmoid & 0.2594 (0.0062) & 0.7220 (0.0098) & 0.2637 (0.0374) & 0.2029 (0.0118) & 0.8280 (0.0128) & 0.4358 (0.0585)\\
tanh & 0.2648 (0.0124) & 0.7273 (0.0050) & 0.2707 (0.0138) & 0.2025 (0.0151) & 0.8171 (0.0151) & 0.4415 (0.0532)\\
relu & 0.2601 (0.0107) & 0.7326 (0.0133) & 0.2546 (0.0109) & 0.2083 (0.0124) & 0.8166 (0.0211) & 0.4100 (0.0276)\\
sigmoid$_{mlp}$ & 0.2836 (0.0102) & 0.5520 (0.0136) & 0.1207 (0.0145) & 0.2127 (0.0294) & 0.7718 (0.0826) & 0.3547 (0.1208)\\
tanh$_{mlp}$ & 0.2587 (0.0121) & 0.7215 (0.0188) & 0.2671 (0.0257) & 0.2024 (0.0181) & 0.8080 (0.0258) & 0.4290 (0.0510)\\
relu$_{mlp}$ & 0.2650 (0.0088) & 0.7205 (0.0122) & 0.2463 (0.0148) & 0.2144 (0.0202) & 0.7993 (0.0212) & 0.3872 (0.0476)\\
Med2Vec & 0.2601 (0.0186) & 0.7447 (0.0194) & \textbf{0.2771} (0.0288) & 0.2044 (0.0129) & 0.8325 (0.0254) & 0.3813 (0.0240)\\
GRAM & 0.2554 (0.0254) & \textbf{0.7586} (0.0240) & 0.2633 (0.0521) & 0.2333 (0.0362) & 0.7785 (0.0260) & 0.3998 (0.0628)\\
\mname & \textbf{0.2535} (0.0042) & 0.7433 (0.0127) & 0.2637 (0.0326) & \textbf{0.1931} (0.0140) & \textbf{0.8393} (0.0281) & \textbf{0.4685} (0.0432)\\
\mname$_{aux}$ & \textbf{0.2512} (0.0073) & \textbf{0.7449} (0.0117) & \textbf{0.2750} (0.0326) & \textbf{0.1910} (0.0163) & \textbf{0.8437} (0.0244) & \textbf{0.4787} (0.0434)\\
\hline
\end{tabular}
}
\end{table*}

==> tables/exp1_table_short_old.tex <==
\begin{table*}[ht]
\caption{HF prediction performance on small datasets. 
Values in the parentheses denote standard deviations from 5-fold random data splits.
All models used GRU for mapping the visit embeddings $\vb^{(1)}, \ldots, \vb^{(T)}$ to a patient representation $\hb$.
Two best values in each column are marked in bold.
A full table with all baselines is provided in Appendix~\ref{appendix:exp1_full}.}
\label{table:exp1}
% \small
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{l|c|c|c|c|c|c}
 & \multicolumn{3}{c|}{\textbf{D$_1$ (Visit complexity 0-15\%, 5608 patients)}} & \multicolumn{3}{c}{\textbf{D$_3$ (Visit complexity 30-100\%, 5231 patients)}}\\
\hline
& test loss & test ROC-AUC & test PR-AUC & test loss & test ROC-AUC & test PR-AUC \\
\hline
raw & 0.2553 (0.0084) & 0.7424 (0.0153) & 0.2669 (0.0314) & 0.2144 (0.0127) & 0.8130 (0.0315) & 0.3776 (0.0589)\\
linear & 0.2562 (0.0108) & 0.7298 (0.0187) & 0.2722 (0.0354) & 0.2021 (0.0176) & 0.8209 (0.0130) & 0.4339 (0.0411)\\
%sigmoid & 0.2594 (0.0062) & 0.7220 (0.0098) & 0.2637 (0.0374) & 0.2029 (0.0118) & 0.8280 (0.0128) & 0.4358 (0.0585)\\
tanh & 0.2648 (0.0124) & 0.7273 (0.0050) & 0.2707 (0.0138) & 0.2025 (0.0151) & 0.8171 (0.0151) & 0.4415 (0.0532)\\
%relu & 0.2601 (0.0107) & 0.7326 (0.0133) & 0.2546 (0.0109) & 0.2083 (0.0124) & 0.8166 (0.0211) & 0.4100 (0.0276)\\
%sigmoid$_{mlp}$ & 0.2836 (0.0102) & 0.5520 (0.0136) & 0.1207 (0.0145) & 0.2127 (0.0294) & 0.7718 (0.0826) & 0.3547 (0.1208)\\
tanh$_{mlp}$ & 0.2587 (0.0121) & 0.7215 (0.0188) & 0.2671 (0.0257) & 0.2024 (0.0181) & 0.8080 (0.0258) & 0.4290 (0.0510)\\
%relu$_{mlp}$ & 0.2650 (0.0088) & 0.7205 (0.0122) & 0.2463 (0.0148) & 0.2144 (0.0202) & 0.7993 (0.0212) & 0.3872 (0.0476)\\
Med2Vec & 0.2601 (0.0186) & 0.7447 (0.0194) & \textbf{0.2771} (0.0288) & 0.2044 (0.0129) & 0.8325 (0.0254) & 0.3813 (0.0240)\\
GRAM & 0.2554 (0.0254) & \textbf{0.7586} (0.0240) & 0.2633 (0.0521) & 0.2333 (0.0362) & 0.7785 (0.0260) & 0.3998 (0.0628)\\
\mname & \textbf{0.2535} (0.0042) & 0.7433 (0.0127) & 0.2637 (0.0326) & \textbf{0.1931} (0.0140) & \textbf{0.8393} (0.0281) & \textbf{0.4685} (0.0432)\\
\mname$_{aux}$ & \textbf{0.2512} (0.0073) & \textbf{0.7449} (0.0117) & \textbf{0.2750} (0.0326) & \textbf{0.1910} (0.0163) & \textbf{0.8437} (0.0244) & \textbf{0.4787} (0.0434)\\
\hline
\end{tabular}
}
\end{table*}

==> tables/exp2_table_short.tex <==
\begin{table*}[ht]
\caption{Test PR-AUC of HF prediction for increasing data size. Parentheses denote standard deviations from 5-fold random data splits. The best value in each column are marked bold.}
\label{table:exp2}
\small
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{l|c|c|c|c}
 %& \multicolumn{3}{c|}{\textbf{E$_1$ (Max. \# of visits 10, 6299 patients)}} & \multicolumn{3}{c}{\textbf{E$_2$ (Max. \# of visits 20, 15794 patients)}}\\
& \textbf{E$_1$ (6299 patients)} & \textbf{E$_2$ (15794 patients)} & \textbf{E$_3$ (21128 patients)} & \textbf{E$_4$ (27428 patients)}\\
\hline
%& test loss & test ROC-AUC & test PR-AUC & test loss & test ROC-AUC & test PR-AUC \\
%\hline
raw & 0.2374 (0.0514) & 0.3149 (0.0367) & 0.3816 (0.0290) & 0.4865 (0.0219)\\
linear & 0.2303 (0.0467) & 0.3200 (0.0353) & 0.3806 (0.0271) & 0.4939 (0.0159)\\
%sigmoid & 0.2354 (0.0355) & 0.3260 (0.0392) & 0.3851 (0.0235) & 0.4823 (0.0195)\\
tanh & 0.2192 (0.0407) & 0.3235 (0.0441) & 0.3884 (0.0310) & 0.4973 (0.0262)\\
%relu & 0.2293 (0.0459) & 0.3274 (0.0359) & 0.3793 (0.0291) & 0.4957 (0.0160)\\
%sigmoid$_{mlp}$ & 0.0843 (0.0154) & 0.0919 (0.0110) & 0.1333 (0.0047) & 0.2221 (0.0146)\\
tanh$_{mlp}$ & 0.2462 (0.0675) & 0.3333 (0.0387) & 0.3834 (0.0209) & 0.4847 (0.0172)\\
%relu$_{mlp}$ & 0.2353 (0.0335) & 0.3111 (0.0494) & 0.3976 (0.0235) & 0.4983 (0.0229)\\
Med2Vec & 0.2404 (0.0228) & 0.3057 (0.0508) & 0.3861 (0.0343) & 0.4756 (0.0148)\\
%GRAM & 0.2292 (0.0570) & 0.3282 (0.0235) & 0.3986 (0.0133) & 0.4893 (0.0073)\\
GRAM & 0.2349 (0.0424) & 0.3118 (0.0337) & 0.4002 (0.0113) & 0.4936 (0.0199)\\
\mname & 0.2711 (0.0308) & 0.3589 (0.0533) & 0.4041 (0.0231) & 0.5129 (0.0204)\\
\mname$_{aux}$ & \textbf{0.2831} (0.0425) & \textbf{0.3651} (0.0473) & \textbf{0.4047} (0.0276) & \textbf{0.5142} (0.0210)\\
\hline
\end{tabular}
}
\end{table*}

==> tables/general_pred.tex <==
\begin{table*}[ht]
\caption{Prediction Performance on Benchmark Tasks. The two strongest performances are marked in bold.}
\label{table:general_pred}
% \small
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{l|c|c|c|c|c|c|c}
 & \multicolumn{3}{c|}{\textbf{HF prediction}} & \multicolumn{2}{c|}{\textbf{Seq. Dx prediction}} & \multicolumn{2}{c}{\textbf{Med. prediction}}\\
\hline
& test loss & test ROC-AUC & test PR-AUC & test loss & test recall@5 & test loss & test recall@5 \\
\hline
raw & 0.2665 (0.0094) & 0.8327 (0.0111) & 0.4843 (0.0220) & 7.2121 (0.0319) & 0.5329 (0.0016) & 3.1842 (0.0575) & \textbf{0.8556} (0.0056) \\
linear & 0.2636 (0.0098) & 0.8372 (0.0108) & 0.4927 (0.0147) & 7.1458 (0.0311) & 0.5450 (0.0008) & 3.1644 (0.0504) & \textbf{0.8547} (0.0054) \\
sigmoid & 0.2649 (0.0100) & 0.8351 (0.0137) & 0.4794 (0.0236) & 7.3494 (0.0438) & 0.5110 (0.0054) & 3.1551 (0.0658) & 0.8506 (0.0059) \\
relu & 0.2642 (0.0098) & 0.8358 (0.0096) & 0.4939 (0.0313) & 7.1597 (0.0349) & 0.5439 (0.0005) & \textbf{3.1314} (0.0503) & 0.8541 (0.0055) \\
linear$_m$ & 0.2688 (0.0084) & 0.8325 (0.0104) & 0.4552 (0.0150) & 7.2548 (0.0354) & 0.5304 (0.0020) & 3.1541 (0.0558) & 0.8494 (0.0055) \\
sigmoid$_m$ & 0.2698 (0.0079) & 0.8281 (0.0117) & 0.4525 (0.0259) & 7.5575 (0.0420) & 0.4784 (0.0053) & 3.1919 (0.0393) & 0.8345 (0.0043) \\
relu$_m$ & 0.2651 (0.0092) & 0.8374 (0.0092) & 0.4762 (0.0270) & 7.2714 (0.0318) & 0.5281 (0.0014) & 3.1373 (0.0536) & 0.8509 (0.0034) \\
sigmoid$_{mlp}$ & 0.3334 (0.0065) & 0.6630 (0.0176) & 0.2222 (0.0146) & 8.7886 (0.0257) & 0.2132 (0.0037) & 3.5345 (0.0518) & 0.7975 (0.0066) \\
relu$_{mlp}$ & 0.2656 (0.0083) & 0.8340 (0.0102) & 0.4825 (0.0279) & 7.1487 (0.0346) & \textbf{0.5464} (0.0012) & 3.1933 (0.0479) & 0.8457 (0.0039) \\
med2vec & 0.2677 (0.0070) & 0.8358 (0.0069) & 0.4668 (0.0069) & 7.2429 (0.0283) & 0.5317 (0.0011) & 3.1976 (0.0503) & 0.8455 (0.0067) \\
$\mname_{sum}$ & \textbf{0.2562} (0.0091) & \textbf{0.8503} (0.0100) & \textbf{0.5040} (0.0181) & \textbf{7.1372} (0.0345) & \textbf{0.5463} (0.0017) & \textbf{3.1007} (0.0429) & 0.8529 (0.0030) \\
$\mname_{bp}$ & \textbf{0.2546} (0.0103) & \textbf{0.8505} (0.0118) & \textbf{0.5130} (0.0196) & \textbf{7.1326} (0.0314) & 0.5460 (0.0012) & 3.1351 (0.0437) & 0.8533 (0.0047) \\
\hline
\end{tabular}
}
\end{table*}

==> tables/mtl_data_stat.tex <==
\begin{table}[h]
\caption{Statistics of the smaller dataset}
\label{table:mtl_data_stat}
% \small
\centering
\begin{tabular}{l|c}
%\textbf{Dataset} & \textbf{Anonymous}\\
%\hline
\hline
\# of patients & 3,973 (272 HF cases)\\ 
\# of visits & 22,415\\
Avg. \# of visits per patient & 5.6\\
Avg. observation period & 10 months\\
%\hline
\# of unique codes & 957 (Dx:239, Rx:86, Proc:632)\\
%- \# of unique diagnosis codes & 239\\
%- \# of unique medication codes & 86\\
%- \# of unique procedure codes & 632\\
\hline
Avg. \# of Dx per visit & 2.31 (Max:20)\\
%Max \# of diagnoses per visit & 29\\
%\hline
Avg. \# of Rx per diagnosis & 0.37 (Max:9)\\
%Max \# of medications per diagnosis & 17\\
%\hline
Avg. \# of Proc. per diagnosis & 0.43 (Max:8)\\
%Max \# of procedures per diagnosis & 10\\
\hline
\end{tabular}
\end{table}

==> tables/multitask_learning.tex <==
\begin{table}[t]
\caption{HF prediction performance on a smaller dataset \js{maybe this is the best experiment, but I doubt anyone read it}}
\label{table:auxiliary_pred}
% \small
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{l|c|c|c}
& test loss & test ROC-AUC & test PR-AUC \\
\hline
raw & \textbf{0.2225} (0.0251) & 0.7572 (0.0380) & 0.2920 (0.0825) \\
linear & 0.2227 (0.0195) & 0.7436 (0.0270) & 0.2986 (0.0569) \\
relu & 0.2400 (0.0261) & 0.7403 (0.0254) & 0.2766 (0.0550) \\
relu$_{mlp}$ & 0.2381 (0.0241) & 0.7211 (0.0216) & 0.2539 (0.0643) \\
% model2$_{\lambda=0}$ & 0.2228 (0.0195) & 0.7503 (0.0307) & 0.3007 (0.0557) \\
$\mname_{bp,aux}$ & 0.2243 (0.0256) & \textbf{0.7640} (0.0222) & \textbf{0.3236} (0.0683) \\
% model2$_{\lambda=0.1}$ & 0.2229 (0.0295) & 0.7617 (0.0269) & 0.3181 (0.0602) \\
\hline
\end{tabular}
%}
\end{table}
